What Needs Attention? Prioritizing Drivers of Developers' Trust and Adoption of Generative AI

Generative AI (genAI) tools promise productivity gains, yet miscalibrated trust and usage friction still hinder adoption. Moreover, genAI can be exclusionary, failing to adequately support diverse users. One such aspect of diversity is cognitive diversity, which leads to diverging interaction styles (e.g., a risk-averse developer may gate genAI outputs behind tests/review; a risk-tolerant one may prototype directly/fix issues post-hoc). When an individual's cognitive styles are unsupported, it creates additional usability barriers. Thus, to design tools that developers trust and use, we must first understand which factors shape their trust and intentions to use genAI at work? We developed a theoretical model of developers' trust and adoption of genAI through a large-scale survey (N = 238) conducted at GitHub and Microsoft. Using Partial Least Squares-Structural Equation Modeling (PLS-SEM), we found aspects related to genAI's system/output quality (e.g., presentation, safety/security, performance), functional value (e.g., educational/practical benefits), and goal maintenance (ability to sustain alignment with task goals) significantly influence trust, which, alongside developers' cognitive styles (i.e., risk tolerance, technophilic motivations, computer self-efficacy), affect adoption. An Importance-Performance Matrix Analysis (IPMA) identified high-importance factors where genAI underperforms, revealing targets for design improvement. We bolster these findings by qualitatively analyzing developers' reported challenges and risks of genAI use to uncover why these gaps persist in development contexts. We offer practical guidance for designing genAI tools that support effective, trustworthy, and inclusive developer-AI interactions.

==> sec/psychometric.tex <==
% \vspace{-1mm}
\subsection{Psychometric Analysis of PICSE Framework}
\label{sec:psycho}

Psychometric quality \cite{lord2008statistical, raykov2011introduction} refers to the objectivity, reliability, and validity of an instrument. We primarily used validated instruments in designing the survey. However, since PICSE was not validated, we conducted a psychometric analysis to empirically refine its factor groupings, which were then evaluated for their association with trust (Sec. \ref{sec:Res}). Table \ref{tab:categories_items} presents the factors evaluated in our survey. We performed the analysis using the JASP tool \cite{jasp_website}, adhering to established psychometric procedures \cite{raykov2011introduction, howard2016review, perrig2023trust} as detailed next:

% Statistical analyses were conducted using the open-source JASP tool \cite{jasp_website}. Our analysis confirmed that a four-factor solution is most appropriate, alongside contributing a validated measurement tool for capturing these factors relative to trust. We followed the recommended psychometric procedures \cite{raykov2011introduction, howard2016review, perrig2023trust}, detailed as follows:
% After these psychometric procedures, the result is a validated and empirically refined grouping of factors from the PICSE framework, thus contributing a reliable measurement tool for capturing these trust-related factors.
% 
% Given the qualitative nature of the PICSE framework, the authors suggest that the categories can, and likely must overlap in practice. 
% 
% In the subsequent subsections, we detail the steps involved in the psychometric quality evaluation of PICSE.

% \vspace{-5mm}
% \vspace{-3mm}

\input{table/picse}
\vspace{3mm}

\textit{1) \textbf{Confirmatory Factor Analysis (CFA) -- Original grouping}}: CFA is a statistical technique that examines intercorrelations between items and proposed factors to test whether a set of observed variables align with a pre-determined factor structure~\cite{harrington2009confirmatory}. We assessed whether the PICSE items align with their original five-factor structure (Personal, Interaction, Control, System, and Expectations). The model fit was evaluated using multiple indices: Chi-square test, Root Mean Square Error of Approximation (RMSEA), Comparative Fit Index (CFI), and Tucker-Lewis Index (TLI) \cite{hu1999cutoff}. Indications of a good model fit include 
$p>.05$ for $\chi^2$ test, $\text{RMSEA}<.06$, $\text{SRMR} \leq .08$, and $0.95 \leq \text{CFI, TLI} \leq 1$ \cite{hu1999cutoff}.
% 
We employed robust maximum likelihood estimator (MLE),\footnote{Robust maximum likelihood estimation adjusts for non-normality in data. In general, ``robust" in factor analyses refer to methods and values resilient to deviations from ideal distributional assumptions.} since the data did not meet multivariate normality assumptions, confirmed using Mardia’s test \cite{mardia1970measures} (see supplemental \cite{supplemental}).
As shown in Table \ref{tab:fit_indices}, results from the original five-factor structure did not indicate a good model fit based on RMSEA, SRMR, CFI, and TLI. This was not entirely unexpected given PICSE's conceptual nature \cite{harrington2009confirmatory}.
% which was not empirically rooted in its construction . 
% Additionally, the original authors suggest that these categories often overlap in practice.
Therefore, to identify a more appropriate model of factors, we proceeded with an exploratory factor analysis (EFA), uncovering alternative groupings that might better fit the data.

\textit{2) \textbf{Exploratory Factor Analysis (EFA)}}: Unlike CFA, which relies on an existing a priori expectation of factor structures, EFA identifies the suitable number of latent constructs (factors) and underlying factor structures without imposing a preconceived model \cite{howard2016review}. Given the violation of multivariate normality, we used principal axis factoring (considering factors with eigenvalues$>1$), as recommended for EFA \cite{howard2016review}. We employed oblique rotation, anticipating correlations among the factors. The data met EFA assumptions: significant Bartlett’s test for sphericity ($\chi^2$ (136) = 1633.97, $p < .001$) and an adequate Kaiser-Meyer-Olkin (KMO) test (0.892, $\text{recommended} \geq .60$) \cite{howard2016review}. 
% 
We used both parallel analysis and a scree plot to determine the number of factors \cite{howard2016review}, suggesting an alternate five-factor model explaining 64.6\% of the total variance. However, most of this variance (60.3\%) was accounted for by factors 1, 2, 3, and 5 (22.7, 15.1, 10.6, and 11.9\% respectively), while factor 4 explained only 4.3\%. The factors showed low correlations (0.2-0.3), except for factor 4, which had high correlations with factors 2 (0.625) and 3 (0.524) (see supplemental). Table \ref{tab:factor_loadings} presents the factor loadings, which indicate the extent to which changes in the underlying factor are reflected in the corresponding indicator (survey item). All items loaded well onto their factors with primary $\text{loadings} > 0.5$ (items with loadings below 0.4 should be excluded) \cite{hair2019use}. 
For interpreting communality (i.e., the proportion of an item's variance explained by the common factors in factor analyses), $\text{values} < 0.5$ are considered problematic and not interpretable~\cite{hair2009multivariate}. As shown in Table~\ref{tab:factor_loadings}, the communality values for items I1, I2, E1, and E2 were below 0.5, and as they did not load onto any of the factors, they were excluded from the final model. Items in factor 4 (P1, P2, C1) also had low communality values and were likewise dismissed. Based on these results, we concluded that a four-factor solution was the most appropriate, dropping factor 4 due to its low variance explanation, high correlations with other factors, and low communality. The fit indices in Table \ref{tab:fit_indices} indicate a good model fit, showing that the EFA factor structure better fits the data than the original PICSE grouping in the above CFA analysis.

\input{table/factor-structure}

\textit{3) \textbf{CFA - Alternate grouping}}: In the final step, as is best practice \cite{raykov2011introduction}, we conducted CFA to validate the factor structure identified through EFA. The CFA fit indices in Table~\ref{tab:fit_indices} confirm the EFA-derived four-factor model (RMSEA = 0.048; SRMR = 0.047, CFI = 0.982, TLI = 0.973).
% 
Table~\ref{tab:factor_loadings} outlines the factor structure and corresponding item groupings. Factor 1, labeled \textbf{\textit{System/Output quality}}, includes items S2 through S5 and E3, which relate to the System group (in PICSE) and the style matching of genAI's outputs. Factor 2, labeled \textit{\textbf{Functional value}}, encompasses items I3 and P3, reflecting the educational value and practical advantages of using genAI tools. Factor 3, labeled \textbf{\textit{Ease of use}}, comprises items S1 and C2, addressing the ease of using and integrating genAI in the workflow. Factor 5, labeled \textbf{\textit{Goal maintenance}}, includes a single item, E4, focusing on genAI's maintenance of human goals. The reliability and validity assessments further support the robustness of these constructs (see Sec. \ref{mm-eval}). 
%After these psychometric procedures, the result is a validated and empirically refined grouping of factors from the PICSE framework. We detail the associations of these factors with trust in Sec. \ref{sec:theory} and \ref{sec:Res}.

In summary, the psychometric analysis confirmed that a four-factor solution is most appropriate and provided a validated measurement instrument for capturing these factors.

\input{table/model-fit}

% To preface subsequent sections, these factors were used to more accurately model trust in genAI tools, thus contributing a reliable measurement tool for understanding these factors relative to trust.


% Based on this we posit:
\vspace{1mm}

==> table/factor-structure.tex <==
\vspace{-2mm}
\begin{table}[htbp]
% \footnotesize
\caption{EFA: Factor loadings and communalities ($h2$)}
%Alternate factor structure (EFA):
\label{tab:factor_loadings}
\vspace{-8pt}
% \small
\centering
\begin{tabular}{>{\raggedright\arraybackslash}m{0.6cm} >{\centering\arraybackslash}m{1cm} >{\centering\arraybackslash}m{1cm} >{\centering\arraybackslash}m{1cm} >{\centering\arraybackslash}m{1cm} >{\centering\arraybackslash}m{1cm} >{\centering\arraybackslash}m{0.9cm}}
\hline
Item & Factor 1 & Factor 2 & Factor 3 & Factor 4 & Factor 5 & $h2$ \\
\hline \hline
\rowcolor{gray!30} S2 & 0.655 & & & & & 0.525 \\
S3 & 0.729 & & & & & 0.609 \\
\rowcolor{gray!30} S4 & 0.823 & & & & & 0.623 \\
S5 & 0.638 & & & & & 0.657 \\
\rowcolor{gray!30} E3 & 0.614 & & & & & 0.559 \\
I3 & & 0.941 & & & & 0.779 \\
\rowcolor{gray!30} P3 & & 0.791 & & & & 0.599 \\
S1 & & & 0.739 & & & 0.668 \\
\rowcolor{gray!30} C2 & & & 0.671 & & & 0.607 \\
P1 & & & & 0.613 & & \textcolor{red}{0.418} \\
\rowcolor{gray!30} P2 & & & & 0.539 & & \textcolor{red}{0.367} \\
C1 & & & & 0.517 & & \textcolor{red}{0.312} \\
\rowcolor{gray!30} E4 & & & & & 0.628 & 0.685 \\
I1 & & & & & & \textcolor{red}{0.398} \\
\rowcolor{gray!30} I2 & & & & & & \textcolor{red}{0.481} \\
E1 & & & & & & \textcolor{red}{0.405} \\
\rowcolor{gray!30} E2 & & & & & & \textcolor{red}{0.492} \\
\hline
\end{tabular}
\begin{tablenotes}
  % \scriptsize
  \footnotesize
\item The applied oblique rotation method is promax. Communality values (h2)\textless 0.5 are problematic \cite{hair2009multivariate} and are marked in \textcolor{red}{RED}. Items loaded well (\textgreater 0.5) onto their primary factors without cross-loadings (\textgreater 0.3) onto other factors \cite{hair2019use}; hence their corresponding cells are kept blank.
% \vspace{-2pt}
    \end{tablenotes}
\end{table}


==> table/htmt.tex <==
\begin{table*}[h]
\centering
\caption{Heterotrait-Monotrait ratio of correlations (HTMT) of the model}
\begin{tabular}{lccccccccc}

\hline
 & \textbf{BI} & \textbf{EoU} & \textbf{FV} & \textbf{IP} & \textbf{LS} & \textbf{M} & \textbf{RT} & \textbf{SE} & \textbf{SOQ} \\ \hline
Behav. Intention (BI) &  &  &  &  &  &  &  &  &  \\
Ease of use (EoU) & 0.631 &  &  &  &  &  &  &  &  \\
Functional Value (FV) & 0.779 & 0.611 &  &  &  &  &  &  &  \\
Info Processing (IP) & 0.064 & 0.27 & 0.1 &  &  &  &  &  &  \\
Learning Style (LS) & 0.412 & 0.167 & 0.473 & 0.326 &  &  &  &  &  \\
Motivations (M) & 0.656 & 0.515 & 0.781 & 0.273 & 0.633 &  &  &  &  \\
Risk Tolerance (RT) & 0.664 & 0.366 & 0.561 & 0.127 & 0.517 & 0.791 &  &  &  \\
Self-Efficacy (SE) & 0.528 & 0.509 & 0.536 & 0.27 & 0.372 & 0.698 & 0.505 &  &  \\
System/Output Quality (SOQ) & 0.686 & 0.646 & 0.635 & 0.156 & 0.262 & 0.573 & 0.226 & 0.283 &  \\
Trust (T) & 0.762 & 0.585 & 0.664 & 0.169 & 0.286 & 0.649 & 0.394 & 0.333 & 0.752 \\ \hline
\end{tabular}
\label{table:correlation_matrix}
\end{table*}
